OSCAR: Optimization-Steered Agentic Planning for Composed Image Retrieval

Composed image retrieval (CIR) requires complex reasoning over heterogeneous visual and textual constraints. Existing approaches largely fall into two paradigms: unified embedding retrieval, which suffers from single-model myopia, and heuristic agentic retrieval, which is limited by suboptimal, trial-and-error orchestration. To this end, we propose OSCAR, an optimization-steered agentic planning framework for composed image retrieval. We are the first to reformulate agentic CIR from a heuristic search process into a principled trajectory optimization problem. Instead of relying on heuristic trial-and-error exploration, OSCAR employs a novel offline-online paradigm. In the offline phase, we model CIR via atomic retrieval selection and composition as a two-stage mixed-integer programming problem, mathematically deriving optimal trajectories that maximize ground-truth coverage for training samples via rigorous boolean set operations. These trajectories are then stored in a golden library to serve as in-context demonstrations for online steering of VLM planner at online inference time. Extensive experiments on three public benchmarks and a private industrial benchmark show that OSCAR consistently outperforms SOTA baselines. Notably, it achieves superior performance using only 10% of training data, demonstrating strong generalization of planning logic rather than dataset-specific memorization.

==> sections/new_method_subsection/case_lib.tex <==
\subsection{Case Library for Inference-Time Guidance}
\label{sec:method:case_lib}
Tool-call trajectories produced by Stage~III provide structured and interpretable supervision signals.
We leverage these trajectories to construct a case library that enables efficient inference-time planning by reusing structured decision patterns learned during optimization.


For each training query, Stage~III produces a tool-call trajectory under the fixed two-clause structure, including the selected tool calls, their rewritten queries and top-$k$ parameters, as well as the resulting set composition.
%
% Each trajectory is stored as a case together with an embedding of the query text and the caption of the reference image, which is used for retrieving similar cases during inference.
Each trajectory is stored as a case, paired with an embedding of the query text and the reference image caption.


Given a new query and a reference image caption,
we retrieve a small set of similar cases from the library
based on embedding similarity between the query text and the reference image caption.
The retrieved cases serve as few-shot guidance for the planner,
enabling structured tool-call generation at test time.


